Tractable General Equilibrium

We study Walrasian economies (or general equilibrium models) and their solution concept, the Walrasian equilibrium. A key challenge in this domain is identifying price-adjustment processes that converge to equilibrium. One such process, t\^atonnement, is an auction-like algorithm first proposed in 1874 by L\'eon Walras. While continuous-time variants of t\^atonnement are known to converge to equilibrium in economies satisfying the Weak Axiom of Revealed Preferences (WARP), the process fails to converge in a pathological Walrasian economy known as the Scarf economy. To address these issues, we analyze Walrasian economies using variational inequalities (VIs), an optimization framework. We introduce the class of mirror extragradient algorithms, which, under suitable Lipschitz-continuity-like assumptions, converge to a solution of any VI satisfying the Minty condition in polynomial time. We show that the set of Walrasian equilibria of any balanced economy-which includes among others Arrow-Debreu economies-corresponds to the solution set of an associated VI that satisfies the Minty condition but is generally discontinuous. Applying the mirror extragradient algorithm to this VI we obtain a class of t\^atonnement-like processes, which we call the mirror extrat\^atonnement process. While our VI formulation is generally discontinuous, it is Lipschitz-continuous in variationally stable Walrasian economies with bounded elasticity-including those satisfying WARP and the Scarf economy-thus establishing the polynomial-time convergence of mirror extrat\^atonnement in these economies. We validate our approach through experiments on large Arrow-Debreu economies with Cobb-Douglas, Leontief, and CES consumers, as well as the Scarf economy, demonstrating fast convergence in all cases without failure.

==> figures/convergence_table_opt.tex <==
\begin{table}[hbtp]
   \caption{Theoretical upper bounds (based on \Cref{thm:mirror_extragradient_global_convergence}) and observed Walrasian deviations in Experiments 1--7
   %\amy{why is this called a violation? we are not violating the bound anywhere?} 
   using step sizes that minimize Walrasian deviation. %(regardless of satisfying pathwise Bregman continuity).
   Minimum deviations correspond to the Walrasian deviation of the best iterate, whereas final deviations correspond to the Walrasian deviation of the last iterate. All deviation values fall well below the corresponding loose theoretical upper bounds.} %\salp{}{The best iterate was the last iterate for Experiment 3 only.}
    \label{table:convergence_bounds_opt}
    \begin{center}
        \renewcommand{\arraystretch}{1.1}
        \begin{tabular}{| m{1.25cm} | m{3cm} m{2cm} m{3.5cm} m{3cm}|}
            \hline
            Exp No. & Loose Upper Bound & Step Size & Minimum Deviation & Final Deviation \\ 
            \hline \hline
            1 & $1.28 \times 10^{2}$ & $4.00 \times 10^{0}$ & $7.19 \times 10^{-9}$ & $3.29 \times 10^{-4}$ \\
            2 & $5.25 \times 10^{1}$ & $4.87 \times 10^{0}$ & $1.49 \times 10^{-6}$ & $1.36 \times 10^{-3}$\\
            3 & $2.56 \times 10^{5}$ & $1.00 \times 10^{-3}$ &$2.79 \times 10^{-1}$ & $2.79 \times 10^{-1}$\\
            4 & $3.05 \times 10^{3}$ & $8.39 \times 10^{-2}$ &$5.82 \times 10^{-3}$ & $8.81 \times 10^{-3}$\\
            5 & $1.21 \times 10^{6}$ & $2.12 \times 10^{-4}$ &$2.05 \times 10^{4}$ & $2.12 \times 10^{4}$\\
            6 & $8.52 \times 10^{5}$ & $3.00 \times 10^{-4}$ &$7.78 \times 10^{3}$ & $7.79 \times 10^{3}$\\
            7 & $5.22 \times 10^{4}$ & $4.90 \times 10^{-3}$ & $5.83 \times 10^{-2}$ & $5.85 \times 10^{-2}$\\ \hline
        \end{tabular}
        \renewcommand{\arraystretch}{1.0}
    \end{center}
\end{table}

